From Linear Logic to Cyclic Sharing

We present a translation from Multiplicative Exponential Linear Logic to a simply-typed lambda calculus with cyclic sharing. This translation is derived from a simple observation on the Int-construction on traced monoidal categories. It turns out that the translation is a mixture of the call-by-name CPS translation and the Geometry of Interaction-based interpretation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{T. Ehrhard, M. Fern\'andez, V. de Paiva, L. Tortora de Falco (Eds.):\\ Linearity-TLLA 2018\\
EPTCS 292, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.292.3}{10.4204/EPTCS.292.3}}

